Certification Design for a Competitive Market

Motivated by applications such as voluntary carbon markets and educational testing, we consider a market for goods with varying but hidden levels of quality in the presence of a third-party certifier. The certifier can provide informative signals about the quality of products, and can charge for this service. Sellers choose both the quality of the product they produce and a certification. Prices are then determined in a competitive market. Under a single-crossing condition, we show that the levels of certification chosen by producers are uniquely determined at equilibrium. We then show how to reduce a revenue-maximizing certifier's problem to a monopolistic pricing problem with non-linear valuations, and design an FPTAS for computing the optimal slate of certificates and their prices. In general, both the welfare-optimal and revenue-optimal slate of certificates can be arbitrarily large.

==> conclusion.tex <==
\nicomment{
\section{Conclusion and Avenues for Future Work}\label{sec:conclusion}

\nicomment{
putting this in comment environment so it will disappear when we compile as it's not complete (and not essential to the submission)}

This article considered the design of recommendation for a competitive market. Under a single-crossing conditions, we showed uniqueness of optimal certification thresholds. We reduce the certification design problem to a pricing problem with non-linear valuations, and show that a fully polynomial time approximatio scheme for this problem exists. We show that optimal menus can be arbitrarily large. A policymaker can improve 

We highlight three areas for future work.

A first is a multi-dimensional version of a problem, in which a certification designer chooses upwards closed sets of qualities $q \in \R^d$, sellers choose to get certified, and a competitive market determines prices. Already in two dimensions, this problem captures policy questions regarding the design of optimal environmental certification, for example whether co-benefits of carbon emission reductions should be mandatory. Compare the survey \cite{karlsson2020climate} on the co-benefits of carbon emissions reductions.

A second question relates to a structural understanding of certification levels in revenue maximization. We observed that welfare and revenue-maximization objectives might lead to different outcomes. We also saw in our example that there might be excessively high certification in our model. A question of particular relevance is whether in a rational market inflationary certification, i.e. too many certified goods are possible, or whether excessively demanding certification, are possible from a revenue-maximizing certifier.
}
